The Shapley Value in Database Management

Attribution scores can be applied in data management to quantify the contribution of individual items to conclusions from the data, as part of the explanation of what led to these conclusions. In Artificial Intelligence, Machine Learning, and Data Management, some of the common scores are deployments of the Shapley value, a formula for profit sharing in cooperative game theory. Since its invention in the 1950s, the Shapley value has been used for contribution measurement in many fields, from economics to law, with its latest researched applications in modern machine learning. Recent studies investigated the application of the Shapley value to database management. This article gives an overview of recent results on the computational complexity of the Shapley value for measuring the contribution of tuples to query answers and to the extent of inconsistency with respect to integrity constraints. More specifically, the article highlights lower and upper bounds on the complexity of calculating the Shapley value, either exactly or approximately, as well as solutions for realizing the calculation in practice.

==> references_backup.tex <==
\bibitem{AAAI21}
Arenas,~M., Barcelo,~P., Bertossi,~L. and Monet,~M. \ The Tractability of SHAP-scores over Deterministic and Decomposable Boolean Circuits. Proc. AAAI, 2021.\\

 \bibitem{AAAI21ext}
    Arenas,~M., Barcelo,~P., Bertossi,~L. and Monet,~M. \ The Tractability of SHAP-scores over Deterministic and Decomposable Boolean Circuits.  Extended version of AAAI 2021 paper. \ arXiv 2104.08015, 2021.\\

 \bibitem{lpnmr19} 
 Bertossi,~L. \ Repair-Based Degrees of Database Inconsistency. Proc. LPNMR, 2019, Springer LNCS 11481, pp. 195-209.\\

    \bibitem{deem}
Bertossi,~L., J. Li,~J.,  Schleich,~M., Suciu,~D.  and Vagena,~Z. \ Causality-based Explanation of Classification Outcomes. Proc. 4th International Workshop on ``Data Management for End-to-End Machine Learning" (DEEM) at ACM SIGMOD/PODS, 2020, pp. 6:1-10.\\


\bibitem{Burkart}
Burkart,~N. and Huber,~M.~F. \ A Survey on the Explainability of
Supervised Machine Learning. \ {\em Journal of Artificial Intelligence Research}, 2021, 70:245-317.\\

 \bibitem{Chockler04}
 Chockler, H.  and Halpern, J.~Y.
\newblock {\it Resp}onsibility and Blame: A Structural-Model Approach.
\newblock {\em Journal of Artificial Intelligence Research}, 2004, 22:93-115.\\

\bibitem{fosca}
Guidotti,~R., Monreale,~A., Ruggieri,~S., Turini,~F., Giannotti,~F. and Pedreschi,~D. \
A Survey of Methods for Explaining Black Box Models. {\em ACM Comput. Surv.}, 51(5):1-93.\\

\bibitem{HP05}
Halpern,~J. and Pearl,~J. \ Causes and Explanations: A Structural-Model Approach. Part I: Causes. \ {\em The
British Journal for the Philosophy of Science}, 2005,
56(4):843-887.\\

 \bibitem{halpern}
Halpern,~J.  {\em Actual Causality}. \  MIT Press, 2016.\\

\bibitem{hunter}
Hunter~A.  and Konieczny,~S. \ On the Measure of Conflicts: Shapley Inconsistency
Values. \ {\em Artificial  Intelligence}, 2010, 174(14):1007–1026.\\

\bibitem{imbens}
Imbens,~G. and Rubin,~D.~B. \ {\em Causal Inference for Statistics, Social, and Biomedical Sciences}. \  Cambridge Univ. Press, 2015.\\

\bibitem{lmcs}
Livshits,~E., Bertossi,~L., Kimelfeld,~B. and Sebag,~M. The Shapley Value of Tuples in Query Answering. {\em Logical Methods in Computer Science}, 2021, 17(3):22.1-22.33.\\

 \bibitem{lund17}
Lundberg,~S. and Lee,~S.-I.  A Unified Approach to Interpreting Model Predictions.  Proc. NIPS, 2017, pp. 4765-4774.\\

\bibitem{lundberg20}
Lundberg, S. M., Erion, G., Chen, H., DeGrave, A., Prutkin, J., Nair, B., Katz, R., Himmelfarb, J., Bansal, N. and Lee, S-I. From Local Explanations to Global Understanding
with Explainable AI for Trees. {\em Nature Machine Intelligence}, 2020, 2(1):56-67.\\

\bibitem{minh}
Minh,~D., Xiang-Wang,~H.,  Fen-Li,~Y. and Nguyen,~T.~N. \  Explainable Artificial Intelligence: A Comprehensive Review.
\ {\em Artificial Intelligence Review}, 2022, 55:3503–3568.\\

\bibitem{molnar}
Molnar,~C.  {\em Interpretable Machine Learning:
A Guide for Making Black Box Models Explainable}, 2020.\\  {\footnotesize https://christophm.github.io/interpretable-ml-book }\\

 \bibitem{pearl}
Pearl,~J. \ {\em Causality: Models, Reasoning and Inference}.  \ Cambridge University Press, 2nd Ed., 2009.\\

\bibitem{roth}
Roth,~A.~E. \ {\em The Shapley Value: Essays in Honor of Lloyd S. Shapley}. Cambridge Univ.
Press, 1988.\\

\bibitem{tapp}
Salimi,~B., Bertossi,~L., Suciu,~D. and Van den Broeck,~G. "Quantifying Causal Effects on Query Answering in Databases". Proc. Theory and Practice of Provenance (TaPP), 2016. \\

\bibitem{Shapley}
Shapley,~L.~S. \ A Value for n-Person Games. \ {\em Contributions to the Theory of Games}, 1953,
2(28):307–317.\\

\bibitem{struss}
Struss,~P. \ Model-Based Problem Solving. \ In {\em Handbook
of Knowledge Representation}, Chap. 4. Elsevier, 2008, pp. 395-465.\\

\bibitem{suciu}
Dan Suciu,~D., Dan Olteanu,~D., Re,~C. and Koch,~C. \ {\em Probabilistic Databases}. Morgan \& Calypool, 2011. 

 \bibitem{guyAAAI21}
Van den Broeck,~G., Lykov,~A., Schleich,~M. and Suciu,~D.  On the Tractability
of SHAP Explanations.  Proc. AAAI, 2021, pp. 6505-6513.
